GlanceVAD: Exploring Glance Supervision for Label-efficient Video Anomaly Detection

In recent years, video anomaly detection has been extensively investigated in both unsupervised and weakly supervised settings to alleviate costly temporal labeling. Despite significant progress, these methods still suffer from unsatisfactory results such as numerous false alarms, primarily due to the absence of precise temporal anomaly annotation. In this paper, we present a novel labeling paradigm, termed "glance annotation", to achieve a better balance between anomaly detection accuracy and annotation cost. Specifically, glance annotation is a random frame within each abnormal event, which can be easily accessed and is cost-effective. To assess its effectiveness, we manually annotate the glance annotations for two standard video anomaly detection datasets: UCF-Crime and XD-Violence. Additionally, we propose a customized GlanceVAD method, that leverages gaussian kernels as the basic unit to compose the temporal anomaly distribution, enabling the learning of diverse and robust anomaly representations from the glance annotations. Through comprehensive analysis and experiments, we verify that the proposed labeling paradigm can achieve an excellent trade-off between annotation cost and model performance. Extensive experimental results also demonstrate the effectiveness of our GlanceVAD approach, which significantly outperforms existing advanced unsupervised and weakly supervised methods. Code and annotations will be publicly available at https://github.com/pipixin321/GlanceVAD.

==> tables/ablation_baseline.tex <==
\begin{table}[!t]
\centering
\caption{Ablation study of different baseline on UCF-Crime and XD-Violence.“$\ast$” represents the results of our implementation.}
\label{table:ablation_baseline}
\vspace{-2mm}
\resizebox{0.75\textwidth}{!}{
\begin{tabular}{l|cc|cc}
\hline\hline
Method  & Params(M) & FLOPS(G) & AUC(\%)$\uparrow$-UCF & AP(\%)$\uparrow$-XD \\
\hline
MIL$^{\ast}$ & 3.15 & 0.63 & 80.83 & 75.24 \\
\textbf{Ours(MIL)} & 3.15 & 0.63 & 87.30$^{\uparrow6.47}$ & 83.61$^{\uparrow8.37}$ \\
\hline
RTFM$^{\ast}$  & 6.18 & 1.24 & 83.50 & 77.53 \\
\textbf{Ours(RTFM)} & 6.18 & 1.24 & 87.80$^{\uparrow4.30}$ & 86.88$^{\uparrow9.35}$ \\
\hline
UR-DMU$^{\ast}$  & 6.30 & 1.31 & 86.54 & 81.47 \\
\textbf{Ours(UR-DMU)}(default) & 6.30 & 1.31 & \textbf{91.96}$^{\uparrow5.42}$ & \textbf{89.40}$^{\uparrow7.93}$ \\
\hline\hline
\end{tabular}
}

\end{table}
